Fault-Tolerant Perception for Automated Driving A Lightweight Monitoring Approach

While the most visible part of the safety verification process of automated vehicles concerns the planning and control system, it is often overlooked that safety of the latter crucially depends on the fault-tolerance of the preceding environment perception. Modern perception systems feature complex and often machine-learning-based components with various failure modes that can jeopardize the overall safety. At the same time, a verification by for example redundant execution is not always feasible due to resource constraints. In this paper, we address the need for feasible and efficient perception monitors and propose a lightweight approach that helps to protect the integrity of the perception system while keeping the additional compute overhead minimal. In contrast to existing solutions, the monitor is realized by a well-balanced combination of sensor checks -- here using LiDAR information -- and plausibility checks on the object motion history. It is designed to detect relevant errors in the distance and velocity of objects in the environment of the automated vehicle. In conjunction with an appropriate planning system, such a monitor can help to make safe automated driving feasible.

==> motivation.tex <==
\section{Motivation}

%\subsection {Previous Work}
%In our previous work \cite{buerkle2020onlineenv} we suggested to realize a monitor architecture comprising RSS, to assure correct behaviour of the planning system,  and a perception monitor using an dynamic occupancy grid.
%
%RSS is a formal mathematical model that describes the safe behaviour of an automated vehicle by mathematical rules. Given a representation of the environment RSS can determine if the current state of the AV is safe or not (according to the RSS definitions). If the state is unsafe, RSS recommends restrictions of the actuator control commands, that should bring the AV back into a safe state. 
%
%To perform its intended function, RSS requires a complete
%and correct environment model containing correct position and velocity of all relevant objects in the surrounding of the vehicle. To assure a correct environment model we proposed an additional RSS Input Validation based on a dynamic occupancy grid. Unfortunately the compute demand creating the dynamic occupancy grid is quite high.
%
%In this paper we want to refine that initial proposal by realizing a monitor for the perception system based on  plausibility checks in combination with less compute intense sensor checks.

\subsection {Monitor}


\begin{figure}
\centering
\includegraphics[width=0.4\textwidth]{images/Architecture2.png}
\caption{Monitor pattern}
\label{fig:Monitor}
\vspace{-0.5cm}
\end{figure}

A monitor architecture [Figure\ref{fig:Monitor}] can be used to assure correct behaviour of a Complex Function. The monitor usually regards the Complex Function as a black box and assures that output of the function is correct. In order to achieve that there are several possibilities:

\begin{itemize}
\item The monitor can utilize information from the input signal and check whether the output of the Complex Function is consistent with the input signal. The input signal could be the same that the Complex Function itself is using or a redundant source of information.
\item Another possibility is to assure that the output of the Complex Function is consistent. This could be checking that the output values are within predefined limits.
Also model knowledge can be utilized. This can be used to check whether the output signal changes are consistent with e.g. physical rules.
\end{itemize} 

It is important to mention that usually not all failures can be detected by a single check. Not all information can be verified by just looking at input data, as usually the purpose of the Complex Function includes interpretation of the input information. Checking correctness of this interpretation just based on the input signal might exceed the capabilities of the monitor.
On the other side just checking consistency of the output signal might not be able to identify permanent failures like, bias of the information or a constant drift.   

\subsection {Monitor for an AV perception system}

As already described the purpose of the monitor is to assure that the input to RSS
is free of safety critical errors. RSS requires as an input an environment model in an object representation. Objects are described by the state $o$ consisting of the position $x,y$, velocity $v_x, v_y$, dimension as bounding box and variance $\Sigma(o)$. Following the argumentation from \cite{buerkle2020onlineenv} absence of errors means that object distance, and therefore object position, and the velocity is correct. 
In an AV the environment model is provided by a perception system, the Complex Function. The perception system receives information from the sensors, e.g. camera, LiDAR and radar, and derives the required object information out of these signals. As already mentioned the required processing is too complex to assure correctness of the provided output. Therefore we want to construct a monitor for this output [Figure\ref{fig:Monitor}], based on the checks described in the previous section.

\begin{itemize}
\item \textbf{Sensor Checks} are correlating sensor information with the object information provided by the perception system. In this work we will make use of LiDAR data.
\item \textbf{Plausibility Checks} will check the consistency of the objects information, by using e.g. model assumptions on the object motion.
\end{itemize} 

As already described the proposed checks are complementary. Not all of the required information can be verified by a single check. LiDAR information can be used to verify position information, but doesn't provide velocity measurements.
In contrast a plausibility check can be used to verified motion of the objects. But might not detect a permanent offset on the object distance.


\subsection{ Availability }

An important aspect that needs to be taken into account is the availability of the end system. The realization of the monitor can have a negative impact, as a false alarm triggered by the monitor might have an impact on the entire AV system and even lead to an necessary emergency manoeuvre. Therefore it is important that the monitor is robust and has a low false alarm rate. This is a design challenge and requires a trade off between sensitivity of error detection capabilities and robustness. Especially as the input to the AV system and therefore the monitor is exposed to noise.




   
  
